DeepSafe: A Data-driven Approach for Checking Adversarial Robustness in Neural Networks

Deep neural networks have become widely used, obtaining remarkable results in domains such as computer vision, speech recognition, natural language processing, audio recognition, social network filtering, machine translation, and bio-informatics, where they have produced results comparable to human experts. However, these networks can be easily fooled by adversarial perturbations: minimal changes to correctly-classified inputs, that cause the network to mis-classify them. This phenomenon represents a concern for both safety and security, but it is currently unclear how to measure a network's robustness against such perturbations. Existing techniques are limited to checking robustness around a few individual input points, providing only very limited guarantees. We propose a novel approach for automatically identifying safe regions of the input space, within which the network is robust against adversarial perturbations. The approach is data-guided, relying on clustering to identify well-defined geometric regions as candidate safe regions. We then utilize verification techniques to confirm that these regions are safe or to provide counter-examples showing that they are not safe. We also introduce the notion of targeted robustness which, for a given target label and region, ensures that a NN does not map any input in the region to the target label. We evaluated our technique on the MNIST dataset and on a neural network implementation of a controller for the next-generation Airborne Collision Avoidance System for unmanned aircraft (ACAS Xu). For these networks, our approach identified multiple regions which were completely safe as well as some which were only safe for specific labels. It also discovered several adversarial perturbations of interest.

==> ACASXu_advs.tex <==
\begin{figure}
%\begin{left}
%\includegraphics[width=4.0in]{figures/Adv1.pdf}
\includegraphics[width=4.0in]{figures/Adv1.png}
\Caption {\footnotesize{Mis-classified as Strong left instead of Strong Right} \label{fig:adv1}}
%\end{left}
\end{figure}

\begin{figure}
%\begin{left}
%\includegraphics[width=4.0in]{figures/Adv2.pdf}
\includegraphics[width=4.0in]{figures/Adv2.png}
\Caption {\footnotesize{Mis-classified as Strong left instead of Strong Right} \label{fig:adv2}}
%\end{left}
\end{figure}

\begin{figure}
%\begin{left}
%\includegraphics[width=4.0in]{figures/Adv3.pdf}
\includegraphics[width=4.0in]{figures/Adv3.png}
\Caption {\footnotesize{Mis-classified as Strong Right instead of Clear of Conflict} \label{fig:adv3}}
%\end{left}
\end{figure}

\begin{figure}
%\begin{left}
%\includegraphics[width=4.0in]{figures/Adv4.pdf}
\includegraphics[width=4.0in]{figures/Adv4.png}
\Caption {\footnotesize{Mis-classified as Strong Right instead of Strong Left} \label{fig:adv4}}
%\end{left}
\end{figure}


==> acmbib.tex <==
\begin{thebibliography}{4}

\bibitem{jour} Smith, T.F., Waterman, M.S.: Identification of Common Molecular
Subsequences. J. Mol. Biol. 147, 195--197 (1981)

\bibitem{lncschap} May, P., Ehrlich, H.C., Steinke, T.: ZIB Structure Prediction Pipeline:
Composing a Complex Biological Workflow through Web Services. In: Nagel,
W.E., Walter, W.V., Lehner, W. (eds.) Euro-Par 2006. LNCS, vol. 4128,
pp. 1148--1158. Springer, Heidelberg (2006)

\bibitem{book} Foster, I., Kesselman, C.: The Grid: Blueprint for a New Computing
Infrastructure. Morgan Kaufmann, San Francisco (1999)

\bibitem{proceeding1} Czajkowski, K., Fitzgerald, S., Foster, I., Kesselman, C.: Grid
Information Services for Distributed Resource Sharing. In: 10th IEEE
International Symposium on High Performance Distributed Computing, pp.
181--184. IEEE Press, New York (2001)

\bibitem{proceeding2} Foster, I., Kesselman, C., Nick, J., Tuecke, S.: The Physiology of the
Grid: an Open Grid Services Architecture for Distributed Systems
Integration. Technical report, Global Grid Forum (2002)

\bibitem{url} National Center for Biotechnology Information, \url{http://www.ncbi.nlm.nih.gov}

\end{thebibliography}


==> figures/Geometry_Horizontal.tex <==
\def\layersep{1.6cm}
\def\layerseP{1.12cm}

\begin{tikzpicture}[scale=0.7]

\node[aircraft top,fill=black,minimum width=1cm,rotate=90,scale = 0.85] (Own) at (0,0) {} node [below,yshift=-0.5cm,font=\footnotesize] {Ownship};
\coordinate[label=right:$v_\text{own}$] (S0) at (0,2.5);

%\coordinate[label=right:£Intruder£] (Int) at (5,5);
\node[aircraft top,fill=black,minimum width=1cm,rotate=166, scale = 0.85] (Int) at (5,2) {};
\node at (5,2) [below,yshift=-0.5cm,font=\footnotesize] {Intruder};
%\node at (5,2) [above,xshift=1.1cm,font=\footnotesize] {Intruder};
\coordinate[label=above:$$] (IntN) at (5,3.6);
\coordinate[label=below:$v_\text{int}$] (S1) at (2.6,2.6);

\coordinate[label=below:$\rho$] (R) at (3.3,1.0);


% arrows
\draw [thick, ->] (Own) -- (S0);
\draw [dashed,->] (Int) -- (IntN);
\draw [thick, ->] (Int) -- (S1);
            
%draw lines
\draw[dashed] (Own) -- (Int);

%angles
\pic [draw,-stealth,red,thick,dashed,angle radius=0.6cm,"$\psi$"{anchor=west,text = black, above}, angle eccentricity=1] {angle = IntN--Int--S1};
\pic [draw,-stealth,red,thick,dashed,angle radius=1.1cm,"$\theta$"{anchor=west,text = black, below}, angle eccentricity=1] {angle = S0--Own--Int};

\end{tikzpicture}

==> futureWrk.tex <==
\section{Future Work}
\label{sec:futureWork}
\label{sec:fw}

Our approach can be extended in several directions that we plan to
pursue in the future.

\begin{enumerate}
    \item{\textbf{Re-training:}} If there are a number of single-input clusters or clusters with low cardinality, it could indicate two cases:
\begin{inparaenum}[(i)]
\item if the density is low, there is not enough training data in that region; or
\item if the density is high, there is a lot of noise or number of redundant attributes, which leads to repeated splitting of clusters.
\end{inparaenum}
 The first case could act as a feedback for re-training. The second
 case is an indicator that the clustering should probably be carried
 out at a higher layer of abstraction, with a smaller number of more
 relevant attributes. 
\item{\textbf{Input to other techniques:}} The boundaries of the
  cluster spheres formed by kMeans lie in low density
  areas. Therefore, the network could be assumed to have low
  accuracy around these boundaries. Thus, adversarial robustness
  checks around instances that are closer to the edge of the
  clusters could exhibit a high number of adversarial perturbations. This analysis
  could help identify potential inputs to which other techniques for
  assessing local robustness could be applied. 
\end{enumerate}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> images.tex <==
\begin{figure}[t]
\begin{center}
\begin{tabular}{c c}
\begin{minipage}[t]{.45\columnwidth}
\includegraphics[width=4.0in]{figures/Adv1.pdf}
\end{minipage}
&
\begin{minipage}[t]{.45\columnwidth}
\includegraphics[width=4.0in]{figures/Adv2.pdf}
\end{minipage}\\
\multicolumn{2}{c}{}
\end{tabular}
\Caption{\footnotesize{(a) Mis-classified as Strong left instead of Strong Right, (b) Mis-classified as Strong left instead of Strong Right} \label{fig:adv1}}
\end{center}
\end{figure} 

==> limit.tex <==
\section{Limitations and Future Extensions}
\noindent{\bf Limitations}.  We next describe some limitations of
\MLR{} in its current form.  \MLR{} has a specific focus on faults in
the branching behavior of the program.  An estimate of the number of
faults in real world programs that belong to this category would help
judge the impact of this approach.

Accuracy of \MLR{} depends on the faulty branch having sufficient
passing test coverage and behavioral diversity. We intend performing
an empirical study of the average ratio of passing to failing tests
coverage of the faulty statement, that are needed to obtain near
accurate results in typical programs.

Accuracy of \MLR{} also relies on an optimal and relevant set of state
predicates to be supplied as features to SVM and decision-tree
learner. As future work, a heuristic selection of predicates such as
based on matching with other parts of the code could be added to the
algorithm.

Assumption that intermediate states for passing executions are correct
since the final output is as expected. Possible ways to mitigate this
would be to perform the semi-supervised learning with an error
threshold for possible noise in the labels of the passing executions.

Despite having representative inputs and ideal labels, decision-trees
could be over-fitted. Specifically when the number of features or
state predicates are high, there could be more than one predicates
having same entropy at a particular level and hence many possible
trees. A possible method to avert this would be to introduce
heuristics in the choice of predicates in the decision-tree learning
algorithm. For instance, predicates with local variables and
expressions with lesser number of de-references could be prioritized
higher than other predicates with the same entropy.

\noindent{\bf Future extensions}.  Potential extensions to \MLR{}
include: (1)~\emph{specification inference} -- \MLR{} could be used to
infer specifications of correct state at different program points;
(2)~\emph{correcting non-branch faults} -- we envisage the use of
multi-class and multi-label learning techniques to correct faults in
statements other than branches; and (3)~\emph{mining data-spectra for
  better fault-localization} -- predicting the behavior of failing
executions based on similar passing executions could help identify
statements which are more likely to be faulty.


==> mnist_Advs.tex <==
\begin{figure}
\begin{center}
\includegraphics[width=4.0in]{figures/MNIST_figs.png}
\Caption {\footnotesize{a) Image of 1 misclassified as 8, b) Image of 1 misclassified as 4, c) Image of 1 misclassified as 3 } \label{fig:image_1_8}}
\end{center}
\end{figure}
\Comment{
\begin{figure}
%\begin{left}
\includegraphics[width=1.0in]{figures/MNIST_INST_1_4.png}
\Caption {\footnotesize{Image of 1 misclassified as 4} \label{fig:image_1_8}}
%\end{left}
\end{figure}

\begin{figure}
%\begin{left}
\includegraphics[width=1.0in]{figures/MNIST_INST_1_4a.png}
\Caption {\footnotesize{Image of 1 misclassified as 4} \label{fig:image_1_8}}
%\end{left}
\end{figure}

\begin{figure}
%\begin{left}
\includegraphics[width=1.0in]{figures/MNIST_INST_1_3.png}
\Caption {\footnotesize{Image of 1 misclassified as 3} \label{fig:image_1_8}}
%\end{left}
\end{figure} 
}
